The evolution of the UV luminosity and stellar mass functions of Lyman-alpha emitters from z~2 to z~6

We measure the evolution of the rest-frame UV luminosity function (LF) and the stellar mass function (SMF) of Lyman-alpha (Lya) emitters (LAEs) from z~2 to z~6 by exploring ~4000 LAEs from the SC4K sample. We find a correlation between Lya luminosity (LLya) and rest-frame UV (M_UV), with best-fit M_UV=-1.6+-0.2 log10(LLya/erg/s)+47+-12 and a shallower relation between LLya and stellar mass (Mstar), with best-fit log10( Mstar/Msun)=0.9+-0.1 log10(LLya/erg/s)-28+-4.0. An increasing LLya cut predominantly lowers the number density of faint M_UV and low Mstar LAEs. We estimate a proxy for the full UV LFs and SMFs of LAEs with simple assumptions of the faint end slope. For the UV LF, we find a brightening of the characteristic UV luminosity (M_UV*) with increasing redshift and a decrease of the characteristic number density (Phi*). For the SMF, we measure a characteristic stellar mass (Mstar*/Msun) increase with increasing redshift, and a Phi* decline. However, if we apply a uniform luminosity cut of log10 (LLya/erg/s) >= 43.0, we find much milder to no evolution in the UV and SMF of LAEs. The UV luminosity density (rho_UV) of the full sample of LAEs shows moderate evolution and the stellar mass density (rho_M) decreases, with both being always lower than the total rho_UV and rho_M of more typical galaxies but slowly approaching them with increasing redshift. Overall, our results indicate that both rho_UV and rho_M of LAEs slowly approach the measurements of continuum-selected galaxies at z>6, which suggests a key role of LAEs in the epoch of reionisation.

==> SC4K_LFs <==
\BOOKMARK [1][-]{section.1}{Introduction}{}% 1
\BOOKMARK [1][-]{section.2}{Sample, photometry and SED fitting}{}% 2
\BOOKMARK [2][-]{subsection.2.1}{The sample: SC4K}{section.2}% 3
\BOOKMARK [2][-]{subsection.2.2}{Multi-wavelength data}{section.2}% 4
\BOOKMARK [2][-]{subsection.2.3}{Multi-wavelength photometry}{section.2}% 5
\BOOKMARK [2][-]{subsection.2.4}{Aperture photometry of SC4K LAEs}{section.2}% 6
\BOOKMARK [2][-]{subsection.2.5}{Spectral Energy Distributions of SC4K LAEs}{section.2}% 7
\BOOKMARK [1][-]{section.3}{The properties of LAEs}{}% 8
\BOOKMARK [2][-]{subsection.3.1}{Ly luminosity \(LLy\)}{section.3}% 9
\BOOKMARK [2][-]{subsection.3.2}{Ly rest-frame equivalent width \(EW0\)}{section.3}% 10
\BOOKMARK [2][-]{subsection.3.3}{Rest-frame UV luminosity \(MUV\)}{section.3}% 11
\BOOKMARK [2][-]{subsection.3.4}{UV continuum slope \(\)}{section.3}% 12
\BOOKMARK [2][-]{subsection.3.5}{Stellar Mass \(M\)}{section.3}% 13
\BOOKMARK [2][-]{subsection.3.6}{Star Formation Rates \(SFRs\)}{section.3}% 14
\BOOKMARK [2][-]{subsection.3.7}{Catalogue of SC4K LAE properties}{section.3}% 15
\BOOKMARK [1][-]{section.4}{Results and Discussion}{}% 16
\BOOKMARK [2][-]{subsection.4.1}{MUV- relation for LAEs and its evolution}{section.4}% 17
\BOOKMARK [2][-]{subsection.4.2}{Implications of MUV- relation for LAEs}{section.4}% 18
\BOOKMARK [2][-]{subsection.4.3}{Ly EW0 and w0: evolution for LAEs?}{section.4}% 19
\BOOKMARK [2][-]{subsection.4.4}{SFR-M relation and evolution}{section.4}% 20
\BOOKMARK [2][-]{subsection.4.5}{LAEs: are they ``Main Sequence" galaxies?}{section.4}% 21
\BOOKMARK [1][-]{section.5}{Conclusions}{}% 22
\BOOKMARK [1][-]{section.A1}{The full SC4K catalogue with PSF photometry and all derived quantities}{}% 23
\BOOKMARK [1][-]{section.A2}{Additional plots and tables}{}% 24

